The impact of resistive electric fields on particle acceleration in reconnection layers

In the context of particle acceleration in high-energy astrophysical environments featuring magnetic reconnection, the importance of the resistive term of the electric field compared to the convective one is still under debate. In this work, we present a quantitative analysis through 2D magnetohydrodynamic numerical simulations of tearing-unstable current sheets coupled to a test-particles approach, performed with the PLUTO code. We find that the resistive field plays a significant role in the early-stage energization of high-energy particles. Indeed, these particles are firstly accelerated due to the resistive electric field when they cross an X-point, created during the fragmentation of the current sheet. If this preliminary particle acceleration mechanism dominated by the resistive field is neglected, particles cannot reach the same high energies. Our results support therefore the conclusion that the resistive field is not only non-negligible but it does actually play an important role in the particle acceleration mechanism.

==> Paper Electric Field/introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
%
%
The study of particle acceleration in astrophysical plasmas such as gamma-ray bursts \citep[GRBs; see, e.g.,][]{Giannios2008, Zhang2011, Sironi2013, Sironi&Giannios2013, Beniamini2014, Beniamini2017}, blazar jets \citep[see, e.g.,][]{Giannios2013, Sironi2015, Petropoulou2016}, supernova remnants \citep[SNRs; see, e.g.,][]{Bell2013, Morlino2013, Caprioli2014} and pulsar wind nebulae \citep[PWNe; see, e.g.,][]{Bucciantini2011,Sironi2011,Cerutti2012,Cerutti2014} is important for the interpretation of the observed spectra of these astrophysical objects. 
Indeed, the investigation of the particle acceleration process would allow a much better understanding of the high energy emission from these objects.

These studies are carried out through numerical simulations, for which several models are available.
On the one hand, Particle-In-Cell (PIC) methods provide the most comprehensive and consistent plasma description at kinetic scales but are inherently limited by resolution constraints fixed by the ion or electron inertial lengths
\citep[see, e.g.,][]{Zenitani2001, Zenitani2008, Jaroschek2004, Lyubarsky2008, Oka2010, Sironi2014, Guo2015, Cerutti2014}.
On the other hand, the magnetohydrodynamic (MHD) model is appropriate for larger scales (i.e., well beyond the particle gyroradius or inertial length) and can be easily coupled to a test-particles approach to investigate acceleration mechanisms \citep[see, e.g.,][]{Onofri2006, Kowal2011, Kowal2012, Zhou2016, Ripperda2017a, Ripperda2017b, Puzzoni2021}.
Test-particles are affected by the electromagnetic field of the plasma but, in turn, do not exert any force on it (no back-reaction), and are often evolved on a fluid snapshot \citep[i.e., where the fluid is frozen in time see, e.g.,][]{Onofri2006, Kowal2011, Kowal2012, Ripperda2017a}.
In this work, conversely, we evolve test-particles along with the fluid \citep[as in, e.g.,][]{Ripperda2017b, Puzzoni2021}.

Of the various acceleration mechanisms, magnetic reconnection is thought to be the most efficient at high magnetizations as it produces power-law spectra of energetic non-thermal particles  \citep[see, e.g.,][]{Zenitani2001, Jaroschek2004, Onofri2006, Bessho2007, Lyubarsky2008, Guo2014, Li2015, Werner2016}.
During the magnetic reconnection process, magnetic energy is converted into thermal and kinetic energy of the plasma as the magnetic field lines of opposite polarity annihilate. 
Magnetic reconnection leads to efficient acceleration when it is triggered by dynamical instabilities such as the tearing mode, during which an initially neutral current sheet fragments into X- and O-points, or plasmoids \citep{Loureiro2016}. 
In the X-points, the magnetic field has null points, while the O-points are characterized by a high current density. 

The orbits followed by the accelerated particles inside the reconnection layer are mainly of the Speiser type \citep[see][]{Speiser1965}, which sample both sides of the current sheet \citep[see, e.g.,][]{Zenitani2001, Giannios2010, Cerutti2013, Zhang2021}.
Particles are accelerated by the plasma electric field, which consists of a convective and a resistive term associated with different acceleration mechanisms. 
Particles can be in fact accelerated directly by the resistive electric field at X-points \citep[see, e.g.,][]{Zenitani2001, Bessho2007, Lyubarsky2008, Sironi2014, Nalewajko2015, Ball2019} or
at the secondary current sheet that forms at the interface between two merging plasmoids \citep[see, e.g.,][]{Oka2010,Sironi2014,Nalewajko2015}.
The energization process can also occur when particles are trapped in a contracting plasmoid due to the Fermi reflection \citep[see, e.g.,][]{Drake2006,Drake2010,Kowal2011,Bessho2012, Petropoulou2018,Hakobyan2021}, associated to the convective electric field.

Which of the two electric field terms dominates in accelerating particles is to date still under debate.
\cite{Kowal2011} and other authors \citep[see, e.g.,][]{Kowal2012,deGouveia2015,delValle2016,Medina2021}, for example, directly neglect the contribution of the resistive field in the particle acceleration mechanism, as they consider it unimportant.
In \cite{Guo2019} and \cite{Paul2021} it is claimed that the Fermi mechanism is the dominant one in the acceleration process, while the crossing of an X-point makes a small contribution to the global energization. 
In particular, \cite{Guo2019} argue that the non-ideal field does not contribute even to the formation of the power-law, but it is only the Fermi mechanism that determines the spectral index.

On the contrary, \cite{Onofri2006} and \cite{Zhou2016} argue that, even if the resistive contribution is less intense than the convective one, it is much more important in accelerating particles. 
The results of \cite{Zhou2016} were later confirmed by \cite{Ripperda2017a}.
In addition, in \cite{Ball2019} it is claimed that the particle acceleration mechanism is more efficient when more X-points are formed.
Recently, \cite{Sironi2022} claimed that the acceleration from the non-ideal electric field is a basic requirement for subsequent acceleration, which is on the contrary typically dominated by the ideal field \citep[as argued by][]{Guo2019}. 
In fact, the particles that do not undergo the non-ideal contribution do not even reach relativistic energies. 

While in \cite{Puzzoni2021} we focused on the problem of convergence concerning the numerical method, here we aim at quantifying the relative importance of the resistive and convective electric field in the particle acceleration process to understand if, when, and why one contribution prevails over the other.
The paper is organized as follows. 
In Section \ref{sec:model} the theoretical and numerical model is explained.
The results are discussed in Section \ref{sec:particle_acceleration}, divided in preliminary considerations made with 2D histograms (\ref{sec:2D_hist}), the study on the importance of the resistive field in accelerating high-energy particles (\ref{sec:res_role}), and the one on the impact of the current sheet evolutionary phases on particle energization (\ref{sec:cs}).
A summary is given in Section \ref{sec:summary}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Paper Electric Field/model.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Theoretical and numerical model}
\label{sec:model}
%
%
Our model follows essentially the same configuration adopted by \cite{Puzzoni2021}, consisting of a perturbed Harris sheet, whose profile is defined by
%
\begin{equation}
  B_x (y) = B_0 \tanh \left(\frac{y}{a}\right),
  \label{eq:B}
\end{equation}
%
where $a = 250 \  c / \omega_p$ denotes the initial width of the current sheet (here $\omega_p$ indicate the plasma frequency).
We normalize the magnetic field strength $B_0$ such that our unit velocity is the Alfv{\'e}n velocity $v_A$, so $\rho_0 = B_0 = 1$ in code units. 
The guide field is absent ($B_z = 0$), and the initial equilibrium is achieved by balancing the Lorenz-force term with a thermal pressure gradient, where the plasma $\beta$ parameter is set to $0.01$ outside the current sheet region,  
%
\begin{equation}
    p(y) = \frac{1}{2} B_0^2 (\beta + 1) - \frac{1}{2} B_x^2 (y)\,.
\end{equation}

Resistive instabilities are triggered by introducing a fixed number of small-amplitudes modes with different wavenumbers $k$.
We achieve this more conveniently by redefining the vector potential according to  $A_z(x,y) = A_0(y) + \delta A_z(x,y)$ where $A_0(y)= a B_0 \log(\cosh(y/a))$ corresponds to the equilibrium magnetic field (equation \ref{eq:B}), while the perturbed term is defined as
%
\begin{equation}
    \delta A_{z}(x,y) = \frac{\epsilon B_0}{N_m} \sum_{m = 0}^{N_m} \frac{1}{k_m} \sin(k_mx + \phi_m) \sech\left(\frac{y}{a}\right),
\end{equation}
%
where $\epsilon = 10^{-3}$ is the perturbation amplitude, $N_m$ is the number of modes \citep[20, as in][]{Puzzoni2021}, $k_m=(m+1)k_0 = 2 \pi (m+1)/L$ are the wavenumbers, and $\phi_m$ are random phases.

We solve the equations of resistive non-relativistic MHD as described in \cite{Puzzoni2021} using the PLUTO code \citep[see][]{Mignone2007, Mignone2012} with the 5$^{\mathrm{th}}$-order WENO-Z reconstruction algorithm \citep[see, e.g.,][]{Borges2008,Mignone2010} in combination with the HLLD Riemann solver of \cite{Miyoshi2005} and the UCT-HLLD emf averaging scheme. 
The redefined Lundquist number $\bar{S}=v_A a/\eta$, corresponding to the current sheet's width $a$, is set to $10^4$. 
The 2D domain is rectangular of size $L \times L/2$ (where $L = 2 \times 10^4 \ c/\omega_p$). 
In the MHD equations, the actual speed of light does not explicitly appear, therefore the artificial value $\mathbb{C} = 10^4 \ v_A$ is used as we want a fluid velocity not comparable to the speed of light. The chosen value of $\mathbb{C}$ can be representative of some astrophysical environments such as coronal mass ejections \citep[CMEs; see, e.g.,][]{Maguire2020} and solar wind \citep[SW; see, e.g.,][]{Bourouaine2012}.
The grid resolution is set to $1536 \times 768$ (i.e. $a/\Delta x \sim 20$) and then progressively doubled up to $6144 \times 3072$ (i.e. $a/\Delta x \sim 80$), in order to determine convergence even in the non-linear evolution phase of the current sheet. 
%\sout{as in \cite{Puzzoni2021} we found that at this resolution the process of particle acceleration already reaches convergence}.

Test-particles are initialized on the grid one per cell and their initial velocities follow a Maxwellian distribution.
Particles obey the equations of motion
%
\begin{equation}\label{eq:particles}
%\syslineskipcoeff{2}
 \begin{dcases} 
  \frac{d \textbf{x}_p}{d t} = \textbf{v}_p \\ 
  \frac{d (\gamma \textbf{v})_p}{d t} = \left(\frac{e}{mc}\right)_p (c \textbf{E} + \textbf{v}_p \times \textbf{B}) \,,
  \end{dcases}
\end{equation}
%
where $\textbf{x}_p$ and $\textbf{v}_p$ represent the spatial coordinate and velocity respectively, $\gamma= (1 - \textbf{v}^2_p/\mathbb{C}^2)^{-1/2}$ is the Lorentz factor while $(e/mc)_p$ is the particle charge to mass ratio. 
The suffix $p$ will be used to label a generic particle.
For computational reasons, the mass of the particles composing the fluid is set equal to that of the accelerated particles.
Consequently, the charge to mass ratio in equation (\ref{eq:particles}) becomes unity when written in code units.

Equation (\ref{eq:particles}) is solved using a standard Boris pusher \citep[see][]{Mignone2018} and the magnetic and electric fields, $\vec{B}$ and $\vec{E}$, are obtained from the fluid.
More specifically, the electric field in resistive MHD is defined by
%
\begin{equation} \label{eq:electricfield}
  c \textbf{E} = - \textbf{v}_g \times \textbf{B} + \frac{\eta}{c} \textbf{J},
\end{equation}
%
where the first term is the convective term ($\textbf{E}_c$) while the second one corresponds to the resistive electric field ($\textbf{E}_r$), where $\eta$ represents the scalar resistivity, assumed constant in this work.
The current density is defined as usual by
%
\begin{equation}\label{eq:currentdensity}
  \textbf{J} = c\nabla \times \textbf{B}
\end{equation}
%
(notice that a constant factor of $\sqrt{4\pi}$ has been reabsorbed in the definition of $\vec{B}$).

In this work, we focus precisely on the relative importance of these two terms in the particle acceleration mechanism.
Each contribution exerts a work on the particles with a corresponding change in their kinetic energy $E_\mathrm{kin} = (\gamma-1)\mathbb{C}^2$.
During a single time step $\Delta t^n$ this variation is given by the sum of the two contributions
%
\begin{equation}
    \Delta E^n_\mathrm{kin} = h^nc
    \left(\textbf{E}_c \cdot \textbf{v}_p + \textbf{E}_r \cdot \textbf{v}_p\right)^n,
    \label{eq:work}
\end{equation}
%
where $h^n =  \Delta t^n(e/mc)_p$ is related to the simulation time step $\Delta t^n$.
In what follows we will make use of the energy gained by the particles which, following equation (\ref{eq:work}), will split into
\begin{equation}
  W =   \sum_n \left(h c \vec{E}_c \cdot \vec{v}_p \right)^n
      + \sum_n \left(h c \vec{E}_r \cdot \vec{v}_p\right)^n \equiv W_c + W_r,
\end{equation}
%
where $n$ indicates the step number.
From now on, (specific) energy and work $W$ will be normalized to $v_A^2$, where $v_A=B_0/\sqrt{\rho_0}$ is the nominal initial Alfv{\'e}n velocity. 



==> Paper Electric Field/results.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results from Numerical Simulations}
\label{sec:particle_acceleration}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}
    \centering
    \includegraphics[width=0.33\textwidth]{Multiple_Hist_CS_S4_1536_78.png}% 
    \includegraphics[width=0.33\textwidth]{Multiple_Hist_CS_S4_3072_78.png}% 
    \includegraphics[width=0.33\textwidth]{Multiple_Hist_CS_S4_6144_78.png}  
    \caption{ 2D histograms of the energy gained (in $\%$) due to the resistive electric field by particles as functions of their kinetic energy at the end of the computational time ($\omega_p t = 7.8 \times 10^5$). The colorbar represents the fraction of particles in each energy bin. The total number of particles in each bin is shown in the corresponding upper panels. These histograms are reproduced at the $N_x = 1536$ (left panels), $N_x = 3072$ (middle panels), and $N_x = 6144$ (right panels) grid resolutions, with $\bar{S} = 10^4$.}
    \label{fig:Hist_2D}
\end{figure*}

%
We performed simulations with $\bar{S}=10^4$ at different grid resolutions to check the convergence properties. 
Moreover, to investigate the importance of the resistive field, numerical computations are carried out twice by first including and then removing the resistive contribution from the equation of motion of the particles, while always keeping it during the fluid evolution.
This means that the fluid evolution is the same in both cases while only the particle evolution differs.

%\sout{the first one in which particles and fluid are evolved together until the end of the computation (co-evolving case, $\omega_p t_\mathrm{stop} = 7.8 \cdot 10^5$), the second one in which particles evolve on a static snapshot of the fluid (stopped at $\omega_p t_\mathrm{snap} \simeq 4.3 \cdot 10^5$), up to the end of the computational time. 
%In the latter case particles remain evenly distributed on the grid until the evolution of the fluid is stopped, from that moment they start moving on this snapshot until the end of the computational time.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preliminary Considerations: 2D Histogram Analysis}
\label{sec:2D_hist}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
While in \cite{Puzzoni2021} we investigated convergence by concentrating on the particle spectra, in this paper, we shift our focus on the convergence properties of the resistive field, by investigating its behaviour at different grid resolutions.
Indeed, a detailed analysis of the resistive contribution is provided by the histograms in Figure \ref{fig:Hist_2D} at the resolution of $N_x = 1536, 3072$ and $6144$ grid zones.
The 2D histograms show the percentage of energy gained by particles due to the resistive electric field at the end of the computational time ($\omega_p t = 7.8 \times 10^5$), as a function of their final kinetic energy.
Notice that a steady state is reached at this time \citep[called \lq\lq saturation phase\rq\rq\ in][]{Puzzoni2021}.
The colors indicate the fraction of particles ($f_\mathrm{part}$) in each energy bin, normalized to the total number of particles in that bin ($N_\mathrm{part}$), which in turn is reported in the corresponding uppermost panels.

As an illustrative example, it is worth looking at the first gray pixel in the first energy bin (lower left corner of the figure) of the middle 2D histogram of Figure \ref{fig:Hist_2D}.
$50\%$ of particles in this energy bin ($N_\mathrm{part} \approx 10^5$, from the corresponding upper panel) is energized between $0-5\%$ by the resistive field.
The corresponding 2D histogram for the convective contribution would be mirrored with respect to the $x$-axis.
Therefore, $50\%$ of particles in the example bin is energized between $95-100\%$ by the convective electric field.

By looking at Fig. \ref{fig:Hist_2D}, the 2D histograms at different grid resolutions show a similar shape. 
The resistive electric field has a small contribution ($W_r \lesssim 30\%$) at low energies ($E_\mathrm{kin} \lesssim 10$).
On the contrary, it has a non-negligible contribution at intermediate energies ($10 \lesssim E_\mathrm{kin} \lesssim 10^3$).
Indeed, up to about $30\%$ of particles are energized up to $100\%$ by the resistive field (see the purple, blue and green pixels).
At high-energies ($E_\mathrm{kin} \gtrsim 10^3$), the resistive contribution slightly decreases with the grid resolution, but still leaves the corresponding energy gain significant.
Indeed, even in the high-resolution case (see rightmost panel), for about $40\%$ of the particles in the last energy bin, the resistive contribution accounts for $40-45\%$ of their energy gain (see orange pixel).
A smaller percentage of particles ($\lesssim 10\%$) are accelerated up to $100\%$ by the resistive field (see purple pixels in the upper right corner).
In the low-resolution case (see leftmost panel), owing to increased numerical diffusion, the amount of work exerted by the resistive electric field is somewhat larger at high-energies ($W_r \gtrsim 50\%$, purple, blue, and green pixels).


Our simulation results indicate that the contribution of the resistive electric field converges with grid resolution at intermediate energies ($10 \lesssim E_\mathrm{kin} \lesssim 10^3$). 
At high energies ($E_\mathrm{kin} \gtrsim 10^3$), however, convergence assessment is somewhat more uncertain, as the contribution of the resistive field appears to decrease as resolution increases.
Further details on plasma convergence are presented in Appendix \ref{app:plasma_convergence}, where we conclude that it was not possible - with the current computational resources - to resolve the typical critical current sheet \citep[i.e., the smallest current layer found in the system; see][]{Uzdensky2010} in the fragmentation phase.
Nevertheless, the resistive contribution is non-negligible at all resolutions. 
Indeed, in the following sections, we will assess its fundamental importance in the particle acceleration mechanism.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The role of the resistive field on high-energy particles}
\label{sec:res_role}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Fig. \ref{fig:hist_1D_br} shows the 1D histograms of the particles kinetic energy at the end of the computational time ($\omega_p t = 7.8 \times 10^5$) for $\bar{S}=10^4$ at different grid resolutions ($N_x = 1536, 3072, 6144$).
The black and the red bars are obtained, respectively, by including or excluding the resistive term in the particle equations of motion.

Following the work of \cite{Sironi2022}, we have decided to remove all the particles that are initially found within the current sheet ($|y_0/a| < 1$) as they have peculiar behavior depending on the initial conditions. 
Moreover, we removed the particles initially farthest from the current sheet ($|y_0/a| > 16$), as they will never reach it within the final simulation time.
This avoids a box size effect or a statistic bias. 
A direct comparison between the two cases clearly indicates that, when the resistive contribution is neglected, the particle spectra are somewhat steeper, characterized by a power-law with index $p \approx 1.8$ at the largest resolutions ($N_x = 3072, 6144$), and the maximum kinetic energy achieved by the particles is lower.
This discrepancy occurs at all resolutions considered here.
For instance, in the $N_x=3072$ case, the maximum kinetic energy achieved by particles by considering the resistive term is $E_\mathrm{kin} \approx 1.3 \times 10^4$, versus the maximum kinetic energy $E_\mathrm{kin} \approx 1.4 \times 10^3$ achieved without including this term.
Similarly, in the $N_x = 6144$ case, the maximum kinetic energy reached by particles is lower when the resistive term is neglected ($E_\mathrm{kin} \approx 4.2 \times 10^3$ versus $E_\mathrm{kin} \approx 1.6 \times 10^4 $).
This confirms, as also argued by \cite{Sironi2022}, that the resistive electric field contribution is fundamental in building the high-energy tail.
As we shall see shortly, this effect takes place in the early stages of the acceleration process.

To this end, we now focus on the resistive contribution in accelerating particles over time and consider only those particles that at the end of the computational time achieved a kinetic energy $E_\mathrm{kin} > E_\mathrm{thr}$. 
We set three different energy threshold: $E_\mathrm{thr} = 10^3, 5 \times 10^3, 10^4$.
For these particles (indicated by the suffix $p$) we calculated the fraction of energy gained due to the resistive contribution, namely $\sum_p W_\mathrm{r, p}/W_\mathrm{tot}$, where $W_\mathrm{tot} = \sum_p W_\mathrm{r,p} + \sum_p W_\mathrm{c,p}$ is the total energy gained by these particles (i.e., also due to the convective contribution).
Fig. \ref{fig:Wr_tot_conf} shows the fractional energy gain of selected particles due to the action of the resistive field as a function of time, for different energy thresholds and for $\bar{S}=10^4$ with a grid resolution $N_x = 3072$ (left panel) and $N_x = 6144$ (right panel).
By looking at this figure, it is clear that the resistive contribution is dominant in accelerating particles at $3.6 \times 10^5 \lesssim \omega_p t \lesssim 4.4 \times 10^5$ for all the kinetic energy thresholds.
Subsequently, the resistive contribution gradually decreases.
In the $N_x = 6144$ case, the resistive contribution towards the end of computational time is lower (see $E_\mathrm{kin} > 5 \times 10^3 \ v_A^2$ and $E_\mathrm{kin} > 10^4 \ v_A^2$).
This result is in agreement with the decline at high-energies observed in the rightmost panel of Figure \ref{fig:Hist_2D}.
Accordingly, if the resistive contribution is removed from the particle equations of motion, particles cannot achieve the same high energies.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relation between particle energization and current sheet evolution}
\label{sec:cs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{\bf Therefore, it is crucial to understand what happens in the current sheet within this time interval.}
Fig. \ref{fig:current_sheet} shows the fluid pressure colored maps at four specific times.
These instants are marked with red points in corresponding lower panels, where we show the resistive field contribution for the particles with final kinetic energies above $E_{\rm thr} =10^3$. 
By looking at the upper left panels ($\omega_p t = 3.4 \times 10^5$), it is clear that the current sheet has reached - in the notations of \cite{Puzzoni2021} - the $2^\mathrm{nd}$- linear phase.
At subsequent times ($\omega_p t = 3.6 \times 10^5$, for instance), the current sheet fragments in X- and O-points (see upper right panel).
This fragmentation phase corresponds to a net increase of the resistive electric field contribution in the particle acceleration mechanism (see corresponding lower panel). 
The increase of the resistive contribution during the fragmentation phase may be explained by the formation of X-points, in which the resistive electric field is strong. 
During the fragmentation phase, plasmoids merge with each other and during this merging process the resistive contribution remains strong, reaching a peak at $\omega_p t = 4.0 \times 10^5$ (see lower left panels).
Indeed, when two plasmoids merge, a secondary current sheet forms at the interface between the two \citep[see, e.g.,][]{Oka2010, Sironi2014, Nalewajko2015}. 
Plasmoids merge until a large final magnetic island is formed.
When major mergers no longer occur, the resistive field contribution begins to smoothly decrease (see lower right panels).
Indeed, towards the end of the computational time, the resistive contribution seems to approach a saturation value, that is when the final giant plasmoid stabilizes \citep[called saturation phase in][]{Puzzoni2021}. 

Therefore, high-energy particles are accelerated by the resistive electric field when they cross an X-point \citep[and are shortly after injected into a plasmoid, see, e.g.,][]{Zenitani2001, Bessho2007, Lyubarsky2008, Sironi2014, Ball2019} and during islands merging. 
When particles are finally trapped inside the large final plasmoid, the resistive contribution decreases, leaving room for the more gradual action of the convective electric field.
These results are in agreement with those of \cite{Sironi2022}, who demonstrated that high-energy particles must have crossed non-ideal regions during the early stages (called \lq\lq injection\rq\rq\  by the author) of their acceleration process.
On the contrary, our results are in contrast with those of \cite{Guo2019}, who claim that the non-ideal field can be neglected in the particle acceleration mechanism, as the Fermi mechanism is the dominant one.
Similarly, our results are different from those of \cite{Kowal2011, Kowal2012} \citep[see also][]{deGouveia2015, delValle2016, Medina2021}, who argue that the resistive contribution is completely negligible in the particle acceleration mechanism.

\begin{figure*}
    \centering
    \includegraphics[width=0.33\textwidth]{hist_1D_S4_1536.png} 
    \includegraphics[width=0.333\textwidth]{hist_1D_S4_3072.png} 
    \includegraphics[width=0.33\textwidth]{hist_1D_S4_6144.png}
    \caption{Histograms of the particles kinetic energy at the end of the computational time ($\omega_p t = 7.8 \times 10^5$) for $\bar{S}=10^4$ at the $N_x = 1536$ (left panel), $N_x = 3072$ (middle panel), and $N_x = 6144$ (right panel) grid resolutions, obtained with (black bars) and without (red bars) the resistive term in the particle equation of motion.}
    \label{fig:hist_1D_br}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.49\textwidth]{Wr_tot_S4_3072.png}
    \includegraphics[width=0.49\textwidth]{Wr_tot_S4_6144.png}
    \caption{ \textit{Left panel}: Resistive contribution over time on particles that at the end of the computational time reach a kinetic energy of $10^3 \ v_A^2$ (green line), $5 \times 10^3 \ v_A^2$ (magenta line), and $10^4 \ v_A^2$ (blue line) for the $\bar{S}= 10^4$ case with a grid resolution $N_x = 3072$. \textit{Right panel}: Same but for $N_x = 6144$. }
    \label{fig:Wr_tot_conf}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{pressure_34.png} 
    \includegraphics[width=0.45\textwidth]{pressure_36.png} \\
    \includegraphics[width=0.45\textwidth]{Wr_tot_S4_3072_34.png} 
    \includegraphics[width=0.45\textwidth]{Wr_tot_S4_3072_36.png} \\
    \includegraphics[width=0.45\textwidth]{pressure_40.png} 
    \includegraphics[width=0.45\textwidth]{pressure_50.png} \\
    \includegraphics[width=0.45\textwidth]{Wr_tot_S4_3072_40.png}
    \includegraphics[width=0.45\textwidth]{Wr_tot_S4_3072_50.png}
    \caption{Resistive field contribution on the most energetic particles ($E_\mathrm{kin} > 10^3$) as a function of time, obtained with $\bar{S}=10^4$ and a grid resolution $N_x = 3072$. This plot is repeated four times being marked with red points, that characterized four evolutionary phases of the current sheet, whose pressure is shown in the corresponding upper panels.}
    \label{fig:current_sheet}
\end{figure*}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Preliminary Considerations}
%\label{sec:1DHistograms}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\sout{The 1D histograms in Figure \ref{fig:hist_156} show the distribution of the time-integrated resistive (in blue) and convective (in red) work done on the particles at the end of the computational time ($\omega_p t = 7.8 \cdot 10^5$) in the snapshot case (upper panel) and in the case where particles and fluid evolve along (middle panel).}
%{\bf The 1D histrograms in Figure \ref{fig:hist_1D} show the distribution of the energy gained by the particles due to the resistive (in blue) and convective (in red) electric field contribution at the end of the computational time ($\omega_p t = 7.8 \cdot 10^5$) for $\bar{S} = 10^3$ (left panel) and for $\bar{S} = 10^4$ (right panel), both with a grid resolution $N_x = 3072$.}
%The histograms only show the positive portion of the work as we have chosen a logarithmic scale.
%Following the work of \cite{Sironi2022} we have \sout{further} decided to remove all the particles that are initially found within the current sheet ($|y_0/a| < 1$) as they have a peculiar behavior depending on the initial conditions. 
%{\bf Moreover, we removed the particles initially farthest from the current sheet ($|y_0/a| > 16$), i.e. those that fail to reach it in computational time, as to avoid a box size effect or a statistics bias.}
%\sout{We obtained the histogram shown in the lower panels of {\bf Figure \ref{fig:hist_1D}} at the end of the computational time ($\omega_p t = 7.8 \cdot 10^5$).}
%{\bf By looking at these histograms it is clear that for $\bar{S}=10^3$ (left panel) the resistive term is not negligible, in particular at high-energies.}
%{\bf In fact, while the two electric field contributions are comparable at low energies, the convective one decreases smoothly as the energy increases.}
%{\bf On the contrary, the high-energy part of the histogram obtained with $\bar{S}=10^4$ (right panel) is dominated by the convective contribution.}
%{\bf However, the resistive contribution is not completely negligible, as it prevails with a peak at intermediate energies (i.e., $10 \lesssim W \lesssim 10^2$).}
%{\bf The contribution of the resistive field has an abrupt cutoff at around $W \sim 4.4 \cdot 10^2$,  while the convective field work decreases more smoothly.}

%\sout{By deleting these particles, the high-energy tail dominated by the convective electric field shown in the middle panel disappears. }
%\sout{This means that the most energized particles at the end of the computational time are those initially found inside the current sheet, and that these are predominantly accelerated by the convective electric field contribution.}

%\sout{By looking at the histograms for both cases it is clear that, even if the high-energy tail is dominated by the convective electric field, the resistive contribution is not negligible in the overall particle energy budget. 
%The most noticeable difference between the two cases is that, in the co-evolving case, particles are less energized.}
%\sout{This should not be surprising as particle acceleration sites and local conditions are dynamically adjusting as fluid elements move.}
%\textbf{\sout{This presumably occurs because a particle in the snapshot case can be bounced back and forth several times between acceleration centers. However, in the time evolving case particle acceleration sites and local conditions are dynamically adjusting as fluid elements move and the scattering centers may be destroyed.}}

%\sout{From the upper panel, we observe a similar trend for the two electric field contributions, with a sharp cutoff at high energies.
%From the middle panel, we notice that in the range $10^2 \lesssim W \lesssim  10^3 $ the two contributions are almost comparable. 
%However, while the contribution of the resistive field has an abrupt cutoff at around $W\sim 2\times 10^3$, the convective field work decreases more smoothly.}


%\begin{figure*}
    %\centering
    %\includegraphics[width=0.45\textwidth]{Hist_S3_3072_CS_156.png}
     %\includegraphics[width=0.45\textwidth]{Hist_S4_3072_CS_156.png}
    %\caption{{\bf {\RED NEW FIGURE!!} \textit{Top panels:} Histogram of the energy gained due to the convective ($W_c$, in red) and resistive ($W_r$, in blue) electric field by the particles at the end of the computational time ($\omega_p t = 7.8 \cdot 10^5$) obtained with $\bar{S}=10^3$ (left panel) and $\bar{S}=10^4$ (right panel) and with a grid resolution $N_x = 3072$.}}
    %\label{fig:hist_1D}
%\end{figure*}

%\begin{figure}
    %\centering
    %\includegraphics[width=0.45\textwidth]{Hist_156_snap.png} 
    %\includegraphics[width=0.45\textwidth]{Hist_156.png} 
    %\includegraphics[width=0.45\textwidth]{Hist_CS_156.png}
    %\caption{\textit{Top panel}: Histogram of the \sout{time-integrated} {\bf energy gained due to the convective ($W_c$, in red) and resistive ($W_r$, in blue) electric field by the particles} evolving on a fluid snapshot at the end of the computational time ($\omega_p t = 7.8 \cdot 10^5$). \textit{Middle panel}: Same as top panel, but for particles evolving along with the fluid. \textit{Bottom panel}: Same as middle panel, but excluding particle initially lying close to the current sheet. }
    %\label{fig:hist_156}
%\end{figure}

%While these 1D histograms provide a semi-quantitative description, their usefulness is limited by the fact that each particle is counted twice as it \sout{contributes to both the resistive and the convective electric field work} {\bf appears both in the $W_c$ bars (i.e., the red bars) and $W_r$ bars (i.e., the blue bars).}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{2D Histrogram Analysis}
%\label{sec:2DHistograms}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}
    %\centering
    %\includegraphics[width=0.45\textwidth]{Multiple_Hist_Snap.png}
    %\caption{ \textit{Top panel}: Histogram of the particles kinetic energy in the snapshot case at the end of the simulation.
    %\textit{Mid and bottom panels}: 2D histograms of the \sout{time-integrated} {\bf energy gained (in $\%$) due to the convective and resistive electric fields, respectively, by the} particles as functions of their final kinetic energy. 
    %The colorbar represents the fraction of particles in each energy bin.}
    %\label{fig:Multiple_Hist_snap}
%\end{figure}
%\begin{figure}
    %\centering
    %\includegraphics[width=0.45\textwidth]{Multiple_Hist.png}
    %\caption{Same of Figure \ref{fig:Multiple_Hist_snap} but for the co-evolving case, at the final simulation time.}
    %\label{fig:Multiple_Hist}
%\end{figure}
%\begin{figure}
    %\centering
    %\includegraphics[width=0.45\textwidth]{Multiple_Hist_CS.png}
    %\caption{Same of Figure \ref{fig:Multiple_Hist} but for particles that are initially found outside the current sheet. The purple dotted line in the top panel represents the fit of the spectrum with a power-law of index {\bf $p = -0.75$}.} 
    %\label{fig:hist_156_CS_2d}
%\end{figure}

%A more detailed analysis is provided by the histograms {\bf in Figures \ref{fig:hist_2D_S3_CS} and \ref{fig:hist_2D_S4_CS} for the $\bar{S} = 10^3$ and $10^4$ cases, respectively} \sout{for the snapshot and co-evolving fluid simulation cases, respectively.}
%The 2D histograms \sout{in the lower and middle panels show, respectively,} {\bf show} the percentage of \sout{time-integrated resistive and convective work} {\bf energy gained by the particles due to the resistive \sout{and convective} electric field as a function of their} kinetic energy at the end of the computational time ($\omega_p t = 7.8 \cdot 10^5$).
%The colors indicate the fraction of particles ($f_\mathrm{part}$) in each energy bin, normalized to the total number of particles in that bin ($N_\mathrm{part}$), in turns reported in the {\bf corresponding} uppermost panels.


%\begin{figure}
    %\centering
    %\includegraphics[width=0.45\textwidth]{Multiple_Hist_Ea_CS_Ideal.png}
    %\caption{Particle energy distribution obtained by excluding the resistive term from the equation of motion. The purple dotted line represents the fit of the spectrum with a power-law of index $p = -1.2$.}
    %\label{fig:hist_ideal}
%\end{figure}

%As an illustrative example, it is worth looking at the last energy bin of {\bf the lower left 2D histrogram of Figure \ref{fig:hist_2D_S4_CS}.} \sout{both figures}.
%{\bf All the particles in this bin ($N_\mathrm{part} = 33$, from the corresponding upper panel) is energized between $30-40\%$ by the resistive field (i.e., the two yellow pixels each corresponding to $50\%$ of the total number of particles in this bin).}
%{\bf The corresponding 2D histogram for the convective contribution would be mirrored with respect to the $x$-axis.}
%\sout{In the snapshot case (Fig. \ref{fig:Multiple_Hist_snap}), all the particles in this bin ($N_\mathrm{part} = 10$, from the upper panel) are energized between $95-100\%$ by the convective field (top right gray pixel in the middle panel) and between $0-5\%$ by the resistive one (bottom right gray pixel in the lower panel).}
%\sout{Likewise, in the co-evolving case (Fig. \ref{fig:Multiple_Hist}), particles in the same energy bin are energized for $90-95\%$ by the convective field and for $5-10\%$ by the resistive one.}

%Thus, by inspecting the 2D histograms {\bf of the $\bar{S}=10^3$ case (see Fig. \ref{fig:hist_2D_S3_CS}), we deduce that at low energies ($0.1 \lesssim W_r \lesssim 10$) about $10\%-20\%$ of the particles are accelerated up to about $20\%$ (i.e., the blue pixels) by the resistive electric field.}
%{\bf This contribution slightly decreases ($0.1 \lesssim W_r \lesssim 1$) at higher resolution ($N_x = 3072$), but a percentage of less than 10\% in this energy range is accelerated up to $100\%$ by the resistive electric field.}
%{\bf On the other hand, at high energies the resistive contribution is strong at all the grid resolutions. }
%{\bf In particular, the gray pixels at $N_x=3072$ (rightmost panel) indicate that the total number of particles in these bins are accelerated for $100\%$ by the resistive term of the electric field.}
%{\bf This result is in agreement with the 1D histogram of the left panel of Figure \ref{fig:hist_1D}, giving us more details.} 
%{\bf Moreover, by looking at the 2D histograms at different grid resolutions, it can be said that the resistive field is \wave{almost} resolved by the $\bar{S}=10^3$ simulations.}
%\sout{in the snapshot case (Fig. \ref{fig:Multiple_Hist_snap}) the convective field is dominant in accelerating the particles, even if a fraction of them ($\sim 10 \%$ of the corresponding bin) is still accelerated only by the resistive field to an energy of $\sim 10^4$.}
%\sout{There is also a small contribution ($W_r \sim 20\%$) in the range $10^5 \lesssim E_\mathrm{kin} \lesssim  10^6 $ for $\sim 20 \%$ of the particles in the corresponding bins.}

%{\bf By looking at the 2D histograms of the $\bar{S}=10^4$ case (see Fig. \ref{fig:hist_2D_S4_CS}) we notice that, even if the spectrum remains substantially the same as the resolution increases (see corresponding upper panels), the resistive contribution trend changes, especially at high energies.}
%{\bf Therefore convergence is not achieved.}
%{\bf The fact that the resistive contribution at high resolutions and energies is weak is in agreement with the right panel of Figure \ref{fig:hist_1D}.}
%{\bf By comparing these histograms with the ones in Figure \ref{fig:hist_2D_S3_CS} it is clear that the resistive contribution at high energies is much lower.}
%{\bf This obviously occurs because at $\bar{S}=10^3$ the physical resistivity is greater compared to that at $\bar{S} = 10^4$. }
%{\bf The only characteristic of the 2D histograms in Figure \ref{fig:hist_2D_S4_CS} that remains similar (since the contribution however decreases as the resolution increases) is the contribution of the resistive field to intermediate energies ($10^2 \lesssim W_r \lesssim 10^3$).}
%{\bf In fact, at lower resolution, about $10-20\%$ of particles are accelerated to these energies for $100\%$ by the resistive field.}
%{\bf However, at high resolution this contribution decreases as it only regards a percentage of particles less than $10\%$.{\RED add numbers}}


%\sout{On  the other hand, in the co-evolving case (Fig. \ref{fig:Multiple_Hist}), the resistive field is not as negligible as in the snapshot case. 
%In fact, in particular, at $10^2 \lesssim E_\mathrm{kin} \lesssim 10^3$ the resistive field contributes the most to the particle acceleration process (i.e. $\sim 20 \%$ of the particles in these bins are accelerated only by this field). 
%We also confirm, as already found by the simpler 1D diagnostic presented in Section \ref{sec:1DHistograms}, that the particle high-energy cutoff is largely overestimated in the snapshot case (see also the upper panel of Fig. \ref{fig:hist_156}).}

%\sout{The 2D histograms reveal that particles starting from outside the current sheet have a sharp cut-off at $E_\mathrm{kin} \approx 6.8 \cdot 10^3 $ and, therefore, do not reach the same high-energy achieved by those initially close to the layer ({\bf $E_\mathrm{kin} \approx 1.6 \cdot 10^4 $}), mainly due to the convective electric field.
%In addition, the presence or absence of these particles changes the 2D histograms. 
%In fact, a direct comparison with Figure \ref{fig:Multiple_Hist} reveals that the acceleration of particles starting within the current sheet is more affected by the resistive contribution at intermediate energies, with a peak at $E_\mathrm{kin} \sim 10^2 $.
%Returning to Figure \ref{fig:hist_156_CS_2d}, we notice that there is a non-negligible contribution of the resistive field at high energies.
%In fact, $\sim 20 \%$ of the particles that reach $E_\mathrm{kin} \approx 4.2 \cdot 10^3 $ are accelerated for about $80 \%$ by the resistive field,  and $\sim 30 \%$ of the particles at $E_\mathrm{kin} \approx 6.8 \cdot 10^3 $ are energized for about $50 \%$ by the same field.
%There is also a contribution at intermediate energies ($10  \lesssim E_\mathrm{kin} \lesssim 10^3$), as $\sim 10 \%$ of the particles in these energy bins are energized by the resistive field for a minimum of about $5 \%$ up to a maximum of approximately $80 \%$ (see the violet pixels in the lower panel). 
%These results further support the idea that the resistive electric field contribution does play a role in the particle acceleration process. }

%\sout{It is alto interesting to note that the spectrum obtained in this case (upper panel) can be fitted with a power-law $dN/d E_\mathrm{kin} \propto E_\mathrm{kin}^{p}$ with slope {\bf $p \approx -0.75$}.}
%\sout{This result is comparable with the one of \cite{Onofri2006}, who found that particles develop a power-law tail of slope $p \simeq -1$.
%\cite{Zenitani2001}, \cite{Jaroschek2004} and \cite{Bessho2007} found a power-law index of about $-1$ in the X-type regions. 
%\cite{Lyubarsky2008} obtained a non-thermal particle spectrum that can be fitted by a power-law with index $p=-1$ and an exponential cutoff.}
%{\bf \sout{Also \cite{Li2015} found that the power-law index approaches $-1$ in the case of non-relativistic reconnection (low-$\beta$ plasma).
%\cite{Guo2014} and \cite{Werner2016} found the same result ($p \approx -1$) but in the relativistic case. 
%These relativistic results are not comparable with our non-relativistic ones, but this work will be extended to the relativistic case in a forthcoming paper.}}

%{\bf The histograms described above show that the contribution of the resistive field is not negligible, but they do not underline its importance in the particle acceleration mechanism.}
%{\bf Therefore}, we have decided to carry out an additional simulation by removing the resistive term from the particles equations of motion, while maintaining the physical resistivity $\eta$ in the MHD equations for the fluid evolution.
%{\bf Figure \ref{fig:hist_nores} shows the comparison between the particle spectra obtained with (upper panels) and without (lower panels) the resistive term in the particle equation of motion for the $\bar{S}=10^3$ (left panels) and $\bar{S}=10^4$ (right panels) case.}
%{\bf These histograms are obtained by filtering the particles as described in the previous paragraph.}
%{\bf By comparing the upper and lower panels it is clear that, when the resistive contribution is neglected, the maximum kinetic energy achieved by the particles is lower: $E_\mathrm{kin} \sim 3.5 \cdot 10^3$ in the lower panel versus $E_\mathrm{kin} \sim 4.2 \cdot 10^4$ in the upper panel for the $\bar{S}=10^3$ case, and $E_\mathrm{kin} \sim 1.4 \cdot 10^3$ in the lower panel versus $E_\mathrm{kin} \sim 6.8 \cdot 10^3$ in the upper panel for the $\bar{S}=10^4$ case.}
%\sout{This yields the 1D histogram shown in Figure \ref{fig:hist_ideal} at the end of the computation, again for the \sout{particles starting from outside the current sheet} {\bf filtered particles shown in Figure \ref{fig:hist_156_CS_2d}}.
%By comparing it with the histogram in the upper panel of Figure \ref{fig:hist_156_CS_2d}, it is clearly noted that the maximum energy achieved is lower ($E_\mathrm{kin} \approx 1.4 \cdot 10^3 $ versus $E_\mathrm{kin} \approx 6.8 \cdot 10^3$ of Fig. \ref{fig:hist_156_CS_2d}), again indicating a non-negligible contribution of the resistive electric field to the high-energy tail .}
%{\bf These results indicate a relevant contribution of the resistive electric field to the high-energy tail.}
%{\bf As already argued in \cite{Sironi2022}, this means that the non-ideal field is fundamental in the particle acceleration early-stages (see Section \ref{sec:time_analysis} for further details) in order to reach high-energies at the end of the computational time.}
%\sout{Besides, the spectrum is now fitted  with a somewhat steeper power-law, with an index $p \approx -1.2$.} {\RED power-law?}
%Our results are, therefore, in contrast with those of \cite{Kowal2011, Kowal2012} \citep[see also][]{deGouveia2015, delValle2016, Medina2021}, who claim that the resistive contribution is completely negligible in the particle acceleration mechanism.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Particle energization over time}
%\label{sec:time_analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Particle energization dependence on initial position and number of X-points}
%\label{sec:initial_Xpoint}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{figure}
    %\centering
    %\includegraphics[width=0.45\textwidth]{E_y.png}\\
    %\includegraphics[width=0.48\textwidth]{Work_Er.png}\\
    %\includegraphics[width=0.48\textwidth]{Work_Ea.png}
    %\caption{\textit{Top panel:} Logarithm of particles final kinetic energy as a function of their initial transverse distance from the current sheet, symmetrically positioned at $y_0=0$ with a thickness $a = 250 \  v_A/\omega_p$.
    %\textit{Middle panel}: Logarithm of the \sout{time-integrated resistive work} {\bf energy gained due to the resistive electric field by the} particles at the end of the computational time in function of their initial position ($x_0, y_0$) on the computational domain. \textit{Bottom panel}: Same but for the \sout{time-integrated resistive work} {\bf convective electric field}.}
    %\label{fig:E_y}
%\end{figure}

%The results of the previous sections indicate that particles initially close to the current sheet are capable of reaching higher energy at the end of the computation.
%This motivates us to investigate how the maximum energy achieved may depend on the particle initial distance from the current sheet.
%The upper panel of Fig. \ref{fig:E_y} shows the relationship between the kinetic energy reached by the particles at the final time ($\omega_p t = 7.8 \cdot 10^5$) and their initial distance from the current sheet (placed at $y_0=0$).
%It can be seen that acceleration becomes less efficient with increasing distance from the sheet, since they fail to reach it in the simulation time.
%Conversely, particles that are initially inside or closer to the current sheet, in particular those at its edges, are the most energized.
%This is confirmed by the middle and lower panel of Figure \ref{fig:E_y}, showing the particles in their initial position on the grid colored according to the logarithm of \sout{the time-integrated resistive and convective work}  {\bf their energy gained through the resistive and convective electric field}, at the end of the computation.
%From the panels, in fact, a sort of stratification is noticed: the closer the particles are initially to the current sheet, the more efficiently they are accelerated, confirming the results of the upper panel.
%This analysis favourably compares to the results of \cite{Zhou2016} and \cite{Nodes2003}.

%We argue that the irregular jagged striped-structure of the energy peaks is due to the non-synchronous arrival time of particles in proximity of the dynamically moving X-points.
%In other words, particles getting energized interact with the newly formed X-points and are accelerated, but not those reaching immediately after since those X-points no longer exist. 
%This depends on the initial distance from the current sheet.
%To prove this statement we have decided to check whether the particles initially lying within a narrow strip around $y_0 \sim 600 \ v_A/\omega_p$, $y_0 \sim 1000 \ v_A/\omega_p$ and $y_0 \sim 2000 \ v_A/\omega_p$ (peaks and thin red stripes in the upper and middle or lower panel of Fig. \ref{fig:E_y}, respectively) enter the current sheet when a large number of X-points is formed.
%This is indeed the case, as shown in Fig. \ref{fig:Xpoints}, where the number of X-points \citep[computed using the same algorithm outlined in][]{Puzzoni2021} is plotted as a function of time.
%The three superimposed red points mark, respectively, the average arrival times of the three selected particles strips in the current sheet.
%It is clear that these instants occur when the number of X-points is around a maximum, thus suggesting a correlation between the efficiency of the acceleration process and the number of formed X-points, as also found by \cite{Ball2019}.

%\begin{figure}
    %\centering
    %\includegraphics[width=0.45\textwidth]{n_xpoints.png}
    %\caption{Number of X-points as a function of time. The three red points represent the instants at which particles starting from $y_0 \sim 600 \ v_A/\omega_p$, $y_0 \sim 1000 \ v_A/\omega_p$, $y_0 \sim 2000 \ v_A/\omega_p$, respectively, enter the current sheet.}
    %\label{fig:Xpoints}
%\end{figure}

%Notice that particles starting from the same $y_0$ stripe are not necessarily energized in the same way. 
%In fact, particles that enter the region of the current sheet that is still in the fragmentation phase, during which the X-points are formed, are accelerated efficiently.
%On the contrary, particles that enter directly the larger magnetic island already formed are less energized.
%This is in agreement with the results of \cite{Lyubarsky2008}, who also divided particles into stripes based on their initial distance from the neutral layer and found that particles passing through an X-point are energized more than those bypassing it.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Individual analysis on two peculiar test-particles}
%\label{sec:single_analyzes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}
    %\centering
    %\includegraphics[width=0.45\textwidth]{Particle_Ekin.png} 
    %\includegraphics[width=0.45\textwidth]{Particle_Work.png} 
    %\caption{\textit{Top panels}: Kinetic energy evolution over time of the most energetic particle starting from inside (solid line) and outside (dashed line) of the current sheet. \textit{Bottom panels}: \sout{Time-integrated resistive (in blue) and convective (in red) work done on} {\bf Energy gained due to the resistive (in blue) and convective (in red) electric field by} the same particles.}
    %\label{fig:particle_Ekin_Work}
%\end{figure}

%We now consider the two most energetic particles that started, respectively, from inside and outside the current sheet, whose initial position along the $y$-axis is, respectively, $y_0 / a \sim -0.8$ and $y_0 / a \sim 8.2$.
%We will label them as the \quotes{innermost} and \quotes{outermost} particle, respectively.
%The upper panel of Figure \ref{fig:particle_Ekin_Work} shows the kinetic energy history of these two particles, while the lower panel shows the corresponding \sout{time-integrated} {\bf energy gained through the convective (in red) and resistive (in blue) electric field}. 
%While the energization of the innermost particle is dominated by the convective electric field, the resistive contribution is of crucial importance in initially accelerating the outermost particle.
%After that, the two contributions tend to become comparable.
%Moreover, the innermost particle is accelerated earlier than the other, thus reaching a higher energy, as reflected by the histograms' high-energy tail.

%\begin{figure*}
    %\centering
    %\includegraphics[width=0.45\textwidth]{Electric_235696.png}\hspace{0.1pt}
    %\includegraphics[width=0.45\textwidth]{Electric_61579.png} \\
    %\caption{Position of the innermost (colored orange in the \textit{left panels}) and outermost (colored green in the \textit{right panels}) on $f_r = |\textbf{E}_r| / (|\textbf{E}_r| + |\textbf{E}_c|)$ in greyscale at two times favorable to their acceleration.}
    %\label{fig:p_evolution}
%\end{figure*}

%The two particles differ not only for their initial position, but also in the acceleration mechanism they are subject to.
%Figure \ref{fig:p_evolution} shows the position of the innermost (left panels) and outermost (right panels) particle, superimposed on $f_r = |\textbf{E}_r| / (|\textbf{E}_r| + |\textbf{E}_c|)$ at two times favorable to their acceleration.
%The innermost particle enters immediately the largest magnetic island (upper left panel) and begins to accelerate. 
%The energization process is due to the $1^{st}$-order Fermi process induced by reflections in the contracting hosting plasmoid that merges with smaller islands and accretes particles as well as magnetic flux \citep[lower left panel; see, e.g.,][]{Drake2006, Drake2010, Kowal2011, Bessho2012, Petropoulou2018, Hakobyan2021}.
%On the other hand, the outermost particle (right panels) enters first a small magnetic island shortly after crossing a X-point (top right panel) and it then undergoes a series of mergers with the other plasmoids until the final coalescence with the largest one (bottom right panel). 
%Just as the particle crosses the X-point and enters the small magnetic island, the \sout{time-integrated work done by} {\bf energy gained due to} the resistive electric field increases sharply (blue dotted line in the lower panel of Fig. \ref{fig:particle_Ekin_Work}), even if the module of the resistive term is $\sim 2\%$ of the total electric field (right panels of Fig. \ref{fig:p_evolution}).
%We point out that the acceleration by X-points is known to be one of the main particle acceleration mechanism that occurs during magnetic reconnection \citep[see, e.g.,][]{Zenitani2001, Bessho2007, Lyubarsky2008, Sironi2014, Nalewajko2015, Ball2019}.

%By inspecting Figure \ref{fig:p_evolution} it can be seen that the resistive field plays a role also at the plasmoids centre as well as at the secondary current sheet that forms perpendicular to the main one at the interface between adjoining plasmoids, where the outermost particle gains further energy \citep[see, e.g.,][]{Oka2010, Sironi2014, Nalewajko2015}.
%Eventually, when the particle becomes trapped in the largest magnetic island, bouncing back and forth, the two electric field contributions tend to be equal. 
%This confirms that the resistive term is crucial in the initial acceleration stages \citep[in agreement with][]{Sironi2022}, and subsequently followed by the action of the convective field \citep[see][]{Guo2019}.

%\begin{figure}
    %\centering
    %\includegraphics[width=0.45\textwidth]{3DTraj_61579.png}
    %\caption{3D trajectory of the outermost particle colored according to the kinetic energy it reaches over time and projected in the $x$-$y$, $x$-$z$ and $y$-$z$ plane respectively. The black symbols are the ones positioned at the times shown in the right panels of Figure \ref{fig:p_evolution}.}
    %\label{fig:orbit}
%\end{figure}

%Finally, the 3D trajectory of the outermost test-particle is shown in Figure \ref{fig:orbit}. 
%The 3D orbit is colored according to the kinetic energy reached by the particle over time, while its projections in the $x$-$y$, $x$-$z$ and $y$-$z$ planes are colored in gray. 
%The black symbols correspond to the times shown in the right panels of Fig. \ref{fig:p_evolution}.
%The trajectory shows oscillations in the $y$-$z$ plane between the two sides of the reconnection layer, thus reminiscent of a Speiser orbit \citep[see][]{Speiser1965}, although the $y$-coordinate increases with time. 
%A similar behavior has been reported by \cite{Zhang2021}, who believe that this effect is due to the interaction with the plasmoid. 
%\uwave{The particle follows a Speiser orbit even in the first moments of acceleration during the merging of the islands after crossing the X-point, but it cannot be seen in this plot as the oscillation is weak and so it would require a zoom.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Paper Electric Field/summary.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Summary}
\label{sec:summary}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this work, we analyzed the role and importance of the resistive electric field in the process of particle acceleration in a reconnecting 2D Harris current sheet.
Our numerical simulations have been carried out with the PLUTO code for plasma astrophysics by simultaneously solving the non-ideal MHD equations with constant resistivity \citep[see][]{Mignone2007, Mignone2012} as well as the motion of test particles.
We choose a Lundquist number $\bar{S}=10^4$, and carry out computations at different grid resolutions ($N_x = 1536, 3072, 6144$).

Our results indicate clear convergence at intermediate energies ($10 \lesssim E_\mathrm{kin} \lesssim 10^3$), while at high energies ($E_\mathrm{kin} \gtrsim 10^3$) convergence achievement is not 
clear–cut.
However, even if the contribution of the resistive field slightly decreases with grid resolution (at high energies), a more detailed analysis reveals that its omission from the particle equations of motion leads to lower (within a factor of $10$) maximum energies and steeper cuts (with a power-law index $p \approx 1.8$ at the largest resolutions) in the particle energy spectra.
This behaviour remains essentially unaffected by grid resolution.

We found that the resistive contribution is strongest as the current sheet starts to fragment and plasmoids start to merge \citep[see][]{Puzzoni2021}.
During this phase, in fact, the resistive contribution sharply increases as a large number of X-points is created (where the resistive electric field is predominant).
The presence of X-points is indeed essential in producing abrupt acceleration of particles at this stage \citep[as found, e.g., by][]{Zenitani2001, Bessho2007, Lyubarsky2008, Sironi2014, Nalewajko2015, Ball2019}.
Moreover, particles energy is boosted also during plasmoids merging, due to the anti-reconnection electric field therein \citep[as demonstrated, e.g., by][]{Oka2010, Sironi2014, Nalewajko2015}. 

The resistive contribution gradually decreases as the system evolves towards the final saturation phase.
Then, as particles are trapped inside the largest magnetic island, they are accelerated by the $1^\mathrm{st}$-order Fermi mechanism in a contracting plasmoid \citep[as found, e.g., by][]{Drake2006, Drake2010, Kowal2011, Bessho2012, Petropoulou2018, Hakobyan2021}, which is dominated by the convective electric field.

In addition, we found particles gaining energy in the core of small plasmoids, where the resistive field is strong.  This is a feature that is missing in PIC simulations \citep[see, e.g.,][]{Petropoulou2018} and it may be an undesirable consequence of a constant resistivity approach. 
Future works will explore different resistivity models that could be more consistent in approaching collisionless plasmas.

Our results lead us to conclude that not only the resistive field is not-negligible \citep[in agreement with the works, for example, of,][]{Onofri2006,Zhou2016, Ball2019,Sironi2022}, but it plays a fundamental role in accelerating high-energy particles.
In particular, our results favourably agree with \cite{Sironi2022}, who argues that the non-ideal field is crucial in the early-stages of particle acceleration.
On the other hand, our outcomes disagree with those of \cite{Kowal2011, Kowal2012}, \cite{deGouveia2015}, \cite{delValle2016} and \cite{Medina2021}, who neglect the resistive electric field in the particle equations of motion as they do not consider it important in the acceleration process.
Similarly, our results also differ from those of \cite{Guo2019}, who argue that the Fermi mechanism is dominant and the non-ideal field can be neglected in the particle acceleration process during large-scale reconnection events, as it is unimportant for the formation of the power-law distribution.

Future simulations will address the issue of longer simulations and different choices of boundary conditions, as well as the extension to the relativistic regime.

